Proxy-Anchor and EVT-Driven Continual Learning Method for Generalized Category Discovery

Continual generalized category discovery has been introduced and studied in the literature as a method that aims to continuously discover and learn novel categories in incoming data batches while avoiding catastrophic forgetting of previously learned categories. A key component in addressing this challenge is the model's ability to separate novel samples, where Extreme Value Theory (EVT) has been effectively employed. In this work, we propose a novel method that integrates EVT with proxy anchors to define boundaries around proxies using a probability of inclusion function, enabling the rejection of unknown samples. Additionally, we introduce a novel EVT-based loss function to enhance the learned representation, achieving superior performance compared to other deep-metric learning methods in similar settings. Using the derived probability functions, novel samples are effectively separated from previously known categories. However, category discovery within these novel samples can sometimes overestimate the number of new categories. To mitigate this issue, we propose a novel EVT-based approach to reduce the model size and discard redundant proxies. We also incorporate experience replay and knowledge distillation mechanisms during the continual learning stage to prevent catastrophic forgetting. Experimental results demonstrate that our proposed approach outperforms state-of-the-art methods in continual generalized category discovery scenarios.

==> related-works/related-works.tex <==
\section{Related Works}
\textbf{Novelty detection} aims to identify samples from novel classes not encountered during the training \textcolor{red}{phase}. 
\textcolor{red}{Methods for novelty detection can be categorized into two main groups of open-set recognition (OSR) and out-of-distribution (OOD) detection. Despite} having small differences, \textcolor{red}{these methods} share the goal of detecting \textcolor{red}{samples} from unknown categories. OOD detection methods include post-hoc, reconstruction, distance-based, density-based, and training-staged approaches. Post-hoc methods do not change the training process \cite{hendrycks2016baseline, liang2017enhancing, hendrycks2019scaling, liu2020energy, sun2021react, sun2022dice}. Reconstruction methods leverage the fact that models trained on ID data cannot effectively compress or reconstruct OOD data \cite{denouden2018improving, jiang2023read}. Distance-based methods use distance measures to ID centroids or prototypes \cite{lee2018simple, sun2022out, wang2022vim, ming2022cider, kim2024neural}. Density-based methods rely on probabilistic modeling to flag samples in low-density regions as OOD \cite{abati2019latent, jiang2021revisiting, zisselman2020deep}. Training-staged methods modify the training process to separate ID and OOD data \cite{hendrycks2018deep, yu2019unsupervised, lee2017training, du2022vos, hsu2020generalized}. 

Open-set recognition methods are categorized as discriminative, generative, or hybrid. Discriminative classifiers are extended to perform open-set recognition either using a distance measure \cite{shu2020p, hassen2020learning, cevikalp2016best} or constructing probability functions for ID/OOD distinction \cite{scherreik2016open, shu2017doc, rudd2017extreme, yoshihashi2019classification, oza2019c2ae}. Generative models create synthetic unknown samples for training \cite{ge2017generative, neal2018open}. Hybrid approaches combine discriminative and generative strategies to learn embeddings jointly \cite{zhang2020hybrid, zhou2021learning, chen2021adversarial}.


\textbf{Category discovery} methods try to identify novel categories within unlabeled data. Early approaches assume that unlabeled data contains only novel \textcolor{red}{samples} and typically follow a multi-stage process, involving pre-training and fine-tuning on labeled and unlabeled data. \textcolor{red}{These} approaches include generating pair-wise pseudo-labels based on feature magnitudes \cite{han2021autonovel, zhao2021novel, zhong2021neighborhood}, clustering unlabeled data using deep embedding clustering \cite{xie2016unsupervised, han2019learning}, and assigning pseudo-labels through self-labeling \cite{joseph2022novel}.

Recent advancements have addressed more realistic scenarios through Generalized Category Discovery (GCD), where unlabeled data includes both previously known and novel classes. GCD \cite{vaze2022generalized} combines self-supervised pre-training, contrastive learning-based fine-tuning, and semi-supervised k-means clustering for novel class discovery. Gaussian mixture model for generalized category discovery
with Protypical Contrastive learning (GPC) \cite{zhao2023learning} employs a semi-supervised Gaussian Mixture Model with prototypical contrastive learning, enabling joint representation learning, cluster estimation, and label assignment without assuming a fixed number of clusters.
In contrast to the multi-stage methods,  UNified Objective function (UNO) \cite{fini2021unified} presents a unified objective function that simultaneously addresses feature extraction, labeled data classification, and clustering of unlabeled data by leveraging pseudo-labels and employing multiple clustering and over-clustering strategies.

\textbf{Continual learning} methods aim to address the challenge of catastrophic forgetting, enabling models to retain previously learned knowledge, while adapting to new tasks. Existing approaches can be broadly categorized into the following: Replay-based techniques focus on mitigating forgetting by storing a subset of previous task data and replaying it during training to reinforce memory of the earlier tasks \cite{chaudhry2019tiny, rolnick2019experience, zheng2024selective, lin2023pcr}. Regularization-based techniques \textcolor{red}{that aim to} preserve prior knowledge by guiding the training process, including parameter regularization to prevent critical parameters from significant updates \cite{kirkpatrick2017overcoming, lee2017overcoming, zenke2017continual, wistuba2023continual}, knowledge distillation, where a "teacher" model transfers knowledge to a "student" model \cite{li2017learning, wu2018memory, hou2019learning}, and data regularization that constrains the optimization process using stored exemplars \cite{lopez2017gradient, chaudhry2018efficient, zhao2023rethinking}. Meta-learning approaches aim to train models capable of rapidly adapting to new tasks with minimal data, leveraging learned algorithms for efficient generalization \cite{finn2017model, gupta2018meta, ostapenko2019learning}. Architecture-based methods address continual learning by modifying or expanding the model’s structure to accommodate new tasks, while preserving existing knowledge \cite{yoon2017lifelong, rusu2016progressive, hu2023dense}. Hybrid methods that use the combination of the aforementioned techniques \cite{li2019learn, wu2021incremental, douillard2020podnet}.

\textbf{Continual generalized category discovery} methods aim to identify novel categories in unlabeled data, which may include both novel \textcolor{red}{samples} and samples from previously known classes. These methods tackle the challenge of discovering new categories incrementally, while retaining knowledge of existing ones.  
Grow and Merge (GM) \cite{zhang2022grow} introduces a framework with two models: a static model that preserves knowledge of old classes and a dynamic model trained \textcolor{red}{in a} self-supervised \textcolor{red}{manner} to discover novel classes. Novel \textcolor{red}{samples} are identified based on their distance to the prototypes of known classes, and the two models are merged, when a new task arrives. Incremental Generalized Category Discovery (IGCD) \cite{zhao2023incremental} employs a non-parametric classifier combined with a density-based exemplar selection method that is employed to select exemplars samples as well discovering novel classes.  
Proxy Anchor (PA) \cite{kim2023proxy} uses proxies learned through proxy anchor loss \cite{kim2020proxy} to detect novel \textcolor{red}{samples}. A non-parametric clustering algorithm clusters and identifies new categories, while catastrophic forgetting is mitigated through experience replay and knowledge distillation. MetaGCD \cite{wu2023metagcd} adopts a meta-learning framework that leverages offline labeled data, to simulate the incremental learning process and utilizes the classic k-means algorithm for novel class discovery. \textcolor{red}{ Happy \cite{ma2024happy} identifies prediction bias and hardness bias as the main challenges in the CGCD scenario, and proposes to address them through clustering-guided initialization and soft entropy regularization for mitigating prediction bias, along with hardness-aware prototype sampling to tackle hardness bias.}
